Excursion Reflected Brownian Motions And Loewner Equations In Multiply Connected Domains

Excursion reflected Brownian motion (ERBM) is a strong Markov process defined in a finitely connected domain $D \subset \C$ that behaves like a Brownian motion away from the boundary of $D$ and picks a point according to harmonic measure from infinity to reflect from every time it hits a boundary component. We give a new construction of ERBM using its conformal invariance and discuss the relationship between the Poisson kernel and Green's function for ERBM and conformal maps into certain classes of finitely connected domains. One important reason for studying ERBM is the hope that it will be a useful tool in the study of SLE in finitely connected domains. To this end, we show how the Poisson kernel for ERBM can be used to derive a Loewner equation for simple curves growing in a certain class of finitely connected domains.

==> OldCopy/Chapter1.tex <==
In order to define excursion reflected Brownian motion, we first need to define excursion measure.  The definition we give is the norm of excursion measure as defined in some references (\cite{MR2129588}, \cite{MR2247843}).  The definition of excursion measure uses the the boundary Poisson kernel $H_{\partial D}(z,w),$ which is the normal derivative of the usual Poisson kernel.  If $z$ is a ``two-sided'' boundary point (an example of this that we will encounter is when $D$ is the upper half plane with a finite number of horizontal slits removed and $z$ is a point in one of the horizontal slits), we should think of $z$ as being two boundary points $z^+$ and $z^-$.  In such cases, for notational convenience we will sometimes write $H_{\partial D}(z,w)$ even when we should consider $H_{\partial D}(z^+,w)$ and $H_{\partial D}(z^-,w)$ separately.  We will adopt a similar convention when considering $H_{\partial D}(z,w)$ or $H_{D}(z,w)$ and $w$ is two-sided.

\begin{definition}
Let $D \subset \C$ be a domain with smooth boundary and let $V$ and $V'$ be disjoint arcs in $\partial D,$ then
\begin{equation*}
\mathcal{E}_D(V,V')=\int_{V}\int_{V'} H_{\partial D}(z,w) \abs{dz}\abs{dw}
\end{equation*}
is called \emph{excursion measure}. Excursion measure normalized to have total mass one is called \emph{normalized excursion measure} and is denoted $\overline{\mathcal{E}}(V,\cdot)$.  
\end{definition}
It is not difficult to check that $\mathcal{E}_D$ is conformally invariant.  This allows us to define $\mathcal{E}_D(V,V')$ even in domains without smooth boundary.  We will often write $\mathcal{E}_D(A,V)$ as shorthand for $\mathcal{E}(\partial A,V)$ and $\overline{\mathcal{E}}(A,V)$ as shorthand for $\overline{\mathcal{E}}(\partial A,V)$.  We will also write $H_{\partial D}(A,z)$ as shorthand for the quantity $\int_{\partial A} H_{\partial D}(z,w) \abs{dz}$.

Let $D=\C \backslash \left[A_0 \cup A_1 \cup \ldots \cup A_n\right]$ where $A_0, A_1, \ldots A_n$ are closed disjoint subsets of $\C$ with $A_i$ larger than a single point for $i\geq 1$ (we allow $A_0$ to be empty), the connected components of $A_0$ simply connected, and $A_1, \ldots A_n$ simply-connected and bounded.  We denote the set of all such domains $\mathcal{Y}$ and all such $n$-connected domains $\mathcal{Y}_n$.  We now give a precise definition of excursion reflected Brownian motion in $D$.  Later we will see that for any $D \in \mathcal{Y}_n$, there is a unique process satisfying the conditions of our definition.

\begin{definition}
\label{characterizationERBM}
Let $E=D\cup\{A_1, \ldots, A_n\}$ equipped with the quotient topology and let $E_{\partial}=E \cup \{A_0\}$ be the one-point compactification of $E$. A stochastic process $B^{ER}_{D}$ with state space $E_{\partial}$ is called an \emph{excursion reflected Brownian motion} (ERBM) if it satisfies the following properties
\begin{enumerate}
\item $B_{D}^{ER}$ has the strong Markov property.

\item If we start the process at $z \in D$ and let
$$T=\inf \{t:  B_{D}^{ER}(t) \in \partial D\},$$
then for $0\leq t \leq T$, $B_{D}^{ER}(t)$ is a Brownian motion in $D$ killed at $\partial D$.

\item Let $\eta_i$ be a smooth Jordan curve in $D$ surrounding $A_i$ (that is, $A_i$ is in the interior of $\eta_i$) and not surrounding $A_j$ for $j\neq i$  and let
$$\sigma=\inf\{t:B_{D}^{ER}(t) \in \eta_i\}$$
be the first time ERBM started at $A_i$ hits $\eta_i$.  Then $B_{D}^{ER}(\sigma)$ has the distribution of $\overline{\mathcal{E}}_{D_i}(A_i,\cdot)$, where $D_i$ is the region bounded by $\partial A_i$ and $\eta_i$.

\item  $B_{D}^{ER}$ is conformally invariant (this will be made more precise in Proposition \ref{ERBMconformalinvariance}) and the radial part of $B_{\C \backslash \D}^{ER}$ has the same distribution as the radial part of reflected Brownian motion in $\C \backslash \D$.
\end{enumerate}
\end{definition}
We will often refer to ERBM in $D$ or $E$ when we really mean the process with the enlarged state space $E_{\partial}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ERBM IN C\D %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Excursion Reflected Brownian Motion in $\C \backslash \D$}
We will now construct ERBM in $E=\C \backslash \D \cup \{\D\}$. We will mimic the construction of Walsh's Brownian motion in \cite{MR1022917}.  The idea of the construction is that if a Feller-Dynkin process exists that satisfies Definition \ref{characterizationERBM}, we can figure out what its semigroup should be.  Once we know what its semigroup should be, we can use general theory to show that there actually is a process with that semigroup.  Finally, once we have the process, we check that it actually satisfies Definition \ref{characterizationERBM}.

Since the radial part of ERBM has the same distribution as the radial part of reflected Brownian motion, to describe the semigroup for ERBM, we use the semigroup for reflected Brownian motion.  There is much in the literature on reflected Brownian motion and it is possible to define it in very general domains.  However, in $\C \backslash \D$ it is possible to give a simple construction.   Let $B_1$ and $B_2$ be independent one-dimensional Brownian motions and define reflected Brownian motion in $\half$ to be the process $B_1+i\abs{B_2}$.  We can then define reflected Brownian motion in $\C \backslash \D$ to be the image of reflected Brownian motion in $\half$ under the map $z \mapsto e^{-iz}$ with the appropriate time change (taking this approach, it is still necessary to check that the resulting process is Feller-Dynkin).
 
\begin{proposition}\label{semigroupERBMThm}
Let $T_t^+$ be the Feller-Dynkin semigroup for reflected Brownian motion in $\C\backslash \D$ and $T_t^0$ be the semigroup for reflected Brownian motion killed when it hits $\D$.  If $f\in C_0(E)$, define an operator $P_t$ by
\begin{equation}
P_t f(r,\theta)=T^+_t \overline{f}(r,\theta)+T_t^0 \paren{f-\overline{f}}(r,\theta),
\label{semigroupERBM}
\end{equation}
where $\displaystyle \overline{f}(r,\theta)=\frac{1}{2\pi} \int_0^{2\pi} f(r,\theta)d\theta.$  If there is a Feller-Dynkin process $B_{\C \backslash \D}^{ER}$ in $\C \backslash \D$ satisfying Definition \ref{characterizationERBM}, its semigroup is $P_t.$
\end{proposition}

\begin{proof}
Let $B_t$ and $R_t$ be respectively Brownian motion and reflected Brownian motion in $\C \backslash \D$ and let $\mathbf{E}$, $\mathbf{E}_1$, and $\mathbf{E}_2$ be the expectations with respect to the probability measures induced by $B_{\C \backslash \D}^{ER}$, $B_t$, and $R_t$ respectively.  Let $\Omega$ be the underlying probability space $B_{\C \backslash \D}^{ER}$, $B_t$, and $R_t$ are defined on and let $\tau$ be the first time $B_{\C \backslash \D}^{ER}$ hits $\D$.  With respect to the appropriate filtration, $\tau$ is a stopping time \cite{MR1796539}.  Finally, let
$$A_t=\{\omega \in \Omega: \tau\leq t\}.$$
By abuse of a notation, we will also denote the set of $\omega$ so that $R_s$ has hit $\D$ by time $t$ and the set of $\omega$ so that $B_s$ has hit $\D$ by time $t$ by $A_t$.  From (2) of Definition \ref{characterizationERBM}, we have that $B_{\C \backslash \D}^{ER}$ is a Brownian motion up until time $\tau$.  From (3) and (4) of Definition \ref{characterizationERBM}, we have that on the set $A_t$, the angular part of $B_{\C \backslash \D}^{ER}$ is uniformly distributed and the radial part is that of reflected Brownian motion.  Combining these facts, we have that if $f\in C_0(E)$, then
\begin{eqnarray*}\displaystyle
P_t f(x)&=& \mathbf{E}^x \paren{f\paren{B_{\C \backslash \D}^{ER}(t)}}\\
&=& \mathbf{E}^x \paren{\mathbf{1}_{A_t}f\paren{B_{\C \backslash \D}^{ER}(t)}}+\mathbf{E}^x \paren{\mathbf{1}_{A_t^c}f\paren{B_{\C \backslash \D}^{ER}(t)}} \\
&=& \mathbf{E}_2^x \paren{\overline{f}\paren{R_t}}+\mathbf{E}_1^x \paren{f\paren{B_t}}-\mathbf{E}_2^x \paren{\mathbf{1}_{A_t^c}\overline{f}\paren{R_t}}-\mathbf{E}_1^x \paren{\mathbf{1}_{A_t}f\paren{B_t}}\\
&=& T_t^+ \overline{f}(x)+T_t^0 f(x)-\mathbf{E}_1^x \paren{\mathbf{1}_{A_t^c}\overline{f}\paren{B_t}}-\mathbf{E}_1^x \paren{\mathbf{1}_{A_t}\overline{f}\paren{B_t}}\\
&=& T^+_t \overline{f}(r,\theta)+T_t^0 \paren{f-\overline{f}}(r,\theta).
\end{eqnarray*}
In the second to last equality, we use the fact that by convention we define $\overline{f}(\D)$ to be $f(\D)$.
\end{proof}

Next we show that $P_t$ as defined in Proposition \ref{semigroupERBM} actually is a Feller-Dynkin semigroup.  We will continue to use the setup given in the beginning of the proof of Proposition \ref{semigroupERBM}.
\begin{proposition}
$P_t$ is a Feller-Dynkin semigroup on $C_0(E)$.  That is,
\begin{enumerate}
\item $P_t: C_0(E) \rightarrow C_0(E)$
\item If $f \in C_0(E)$ and $0 \leq f \leq 1,$ then $0 \leq P_t f \leq 1$.
\item $P_0$ is the identity on $C_0(E)$ and $P_tP_s=P_{t+s}$
\item $\displaystyle \lim_{t \rightarrow 0} \left\| P_t f - f\right\|_{\infty} =0$ for all $f \in C_0(E)$.
\end{enumerate}
\end{proposition}

\begin{proof}
If $f \in C_0(E)$, then $\overline{f}$ is also in $C_0(E)$.  We now have
\begin{eqnarray*}
\abs{P_t f(r,\theta)-P_t f(r',\theta')} &\leq& \abs{T_t^+ \overline{f}(r,\theta) - T_t^+ \overline{f}(r',\theta')}\\
& & +\abs{T_t^0f(r,\theta)-T_t^0f(r',\theta')}\\
& & + \abs{T_t^0\overline{f}(r,\theta)-T_t^0 \overline{f}(r',\theta')}
\end{eqnarray*}
The fact that $P_t f$ is continuous now follows from the fact that $T_t^0 f$, $T_t^0 \overline{f}$, and $T_t^+ \overline{f}$ are all continuous.  Also, since both $f$ and $\overline{f}$ vanish at infinity, so does $P_t f$.  This proves (i).

From the proof of Proposition \ref{semigroupERBM} we have
\begin{eqnarray*}
P_t f(x)&=&\mathbf{E}_2^x \paren{\mathbf{1}_{A_t}\overline{f}(R_t)}+\mathbf{E}_1^x \paren{\mathbf{1}_{A_t^c}f(B_t)}.
\end{eqnarray*}
If $0 \leq f \leq 1$, then
\begin{eqnarray*}
0 &\leq & \mathbf{E}_2^x \paren{\mathbf{1}_{A_t}\overline{f}(R_t)}+\mathbf{E}_1^x \paren{\mathbf{1}_{A_t^c}f(B_t)} \\
&\leq& \mathbf{E}_2^x \paren{\mathbf{1}_{A_t}}+\mathbf{E}_1^x \paren{\mathbf{1}_{A_t^c}}\\
&=& 1.
\end{eqnarray*}
(ii) follows.

It's clear from the corresponding property for $T_t^+$ and $T_t^0$ that $P_0$ is the identity on $C_0(E)$.  Next observe
\begin{eqnarray*}
\overline{P_s f}(r,\theta)&=&\overline{T_s^+ \overline{f}}(r,\theta) + \overline{T_s^0 f}(r,\theta) -\overline{T_s^0\overline{f}}(r,\theta)\\
&=&T_s^+ \overline{f}(r,\theta) + \int_0^{2\pi}T_s^0 f(r,\theta)d\theta -T_s^0 \overline{f}(r,\theta)\\
&=&T_s^+ \overline{f}(r,\theta) + T_s^0 \overline{f}(r,\theta)-T_s^0 \overline{f}(r,\theta)\\ %Fubini?
&=& T_s^+ \overline{f}(r,\theta)
\end{eqnarray*}
and thus
\begin{equation*}
P_s f(r,\theta)- \overline{P_s f}(r,\theta)=T_s^0\paren{f-\overline{f}}(r,\theta).
\end{equation*}
Using these two facts and the fact that (iii) holds for $T_t^+$ and $T_t^0$, we have
\begin{eqnarray*}
P_t P_s f(r,\theta)&=& T_t^+ \overline{P_s f}(r,\theta)+T_t^0\paren{P_s f(r,\theta)- \overline{P_s f}(r,\theta)}\\
&=& T_t^+ T_s^+ \overline{f}(r,\theta)+T_t^0 T_s^0 \paren{f-\overline{f}}(r,\theta)\\
&=&T_{t+s}^+ \overline{f}(r,\theta)+T_{t+s}^0\paren{f-\overline{f}}(r,\theta)\\
&=&P_{t+s} f(r,\theta)
\end{eqnarray*}
This proves (iii).

Since (i)-(iii) hold, by (say) Lemma III.6.7 of \cite{MR1796539}, to prove (iv) it is enough to show that for all $f \in C_0(E)$ we have
$$\displaystyle \lim_{t \rightarrow 0}P_t f(z)=f(z)$$
for all $z\in E$.  Since $T_t^+$ and $T_t^0$ satisfy (i)-(iv), we have
\begin{eqnarray*}
\displaystyle \lim_{t \rightarrow 0} P_t f(z)&=& \lim_{t \rightarrow 0} T_t^+ \overline{f}(z)+\lim_{t \rightarrow 0} T_t^0 \paren{f-\overline{f}}(z)\\
&=&\overline{f}(z)+\paren{f(z)-\overline{f}(z)}\\
&=& f(z),
\end{eqnarray*}
which proves (iv).
\end{proof}

Now using (say) Theorem III.7.1 of \cite{MR1796539}, given any measure $\mu$ on $E$, we can define a unique Feller-Dynkin process
 \begin{equation} \label{ERBMdef}
B^{ER}_{\C\backslash \D}:=\paren{\Omega,\mathscr{F},\{\mathscr{F}_t:t\geq 0\},\{B^{ER}_{\C\backslash \D}(t):t\geq 0\},\{\proj^{\mu}\}}
\end{equation}
with semigroup $P_t$.  Furthermore, the filtration $\mathscr{F}_t$ in independent of the measure $\mu$ and $X$ has the strong Markov property with respect to this filtration.  We denote the angular and radial parts of $B^{ER}_{\C\backslash \D}$ at time $t$ by $\theta_t$ and $R_t$ respectively.

We now check that the process $B^{ER}_{\C\backslash \D}$ defined in (\ref{ERBMdef}) satisfies Definition \ref{characterizationERBM}.
\begin{proposition}
$B^{ER}_{\C \backslash \D}$ killed the first time it hits $\partial \D$ is Brownian motion in $\C\backslash \D$.
\label{ERBMlikeBM}
\end{proposition}
\begin{proof}
Using (\ref{semigroupERBM}), it is clear that the two processes have the same semigroup.
\end{proof}

\begin{proposition} \label{radialpartERBM}
With respect to the filtration $\mathscr{F}_t$ and measure $\mathbf{P}^{\mu}$, $R_t$ is the radial part of reflected Brownian motion in $\C \backslash \D$.
\end{proposition}
\begin{proof}
We mimic the proof of Lemma 2.2 in \cite{MR1022917}.  Let $g \in C_0([1,\infty))$ and define $f \in C_0(E)$ by $f(r,\theta)=g(r).$  Observe that $\overline{f}=f$ and $f(X_t)=g(R_t)$.  If $S$ is any $\mathscr{F}_t$-stopping time, then
\begin{eqnarray*}
\mathbf{E}^{\mu}\paren{g(R_{S+t})|\mathscr{F}_S}&=&\mathbf{E}^{\mu}\paren{f(X_{S+t})|\mathscr{F}_S}\\
&=& P_t f(X_S)\\
&=& T_t^+ \overline{f}(R_S,\theta_S)+T_t^0\paren{f-\overline{f}}(R_S,\theta_S)\\
&=& T_t^+ f (R_S,\theta_S)\\
&=& R_t^+ g(R_S),
\end{eqnarray*}
where $R_t^+$ is the semi-group for the radial part of reflected Brownian motion in $\C \backslash \D$. The result follows.
\end{proof}

\begin{proposition} \label{excursiondistERBM}
Let $\eta$ be a smooth simple curve surrounding $\D$, $B$ be the region bounded by $\eta$ and $\D$, and $\tau$ be the first time $B^{ER}_{\C \backslash \D}$ started at $\D$ leaves $B$.  If $V$ is a smooth sub-arc of $\eta$, then
\begin{equation*}
\alpha:= \proj^{\D} \paren{B^{ER}_{\C \backslash \D}(\tau) \in V}=\overline{\mathcal{E}}_B(\D,V)
\end{equation*}
\end{proposition}

\begin{proof}
Let $C_{\epsilon}$ be the circle of radius $\epsilon$ centered at the origin.  Since it is clear from (\ref{semigroupERBM}) that $B_{\C\backslash \D}^{ER}$ is rotationally invariant, the result follows in the case that $\eta=C_{\epsilon}$ for some $\epsilon$.

Let $p(z)$ be the probability that Brownian motion started at $z$ exits $B$ on $\eta$.  For small enough $\epsilon$, $C_{\epsilon}$ is in the interior of $\eta$.  For such an $\epsilon$, using the strong Markov property and Proposition \ref{ERBMlikeBM}, we see
\begin{eqnarray*}
2\pi \alpha &=& \int_{C_{\epsilon}}\paren{\int_V H_B\paren{z,w} \abs{dw}+\paren{ 1-p(z)}\alpha}\abs{dz} \\
&=& 2 \pi \alpha+ \int_{C_{\epsilon}} \paren{\int_V H_B(z,w) \abs{dw}-p(z)\alpha}\abs{dz}\\
&=& 2 \pi \alpha +\int_{C_{\epsilon}} \paren{\int_V H_B(z,w) \abs{dw}-\alpha\int_{\eta} H_B(z,w)\abs{dw}}\abs{dz}.
\end{eqnarray*}
As a result, for small enough $\epsilon$, we have
$$\displaystyle\alpha=\frac{\int_{C_{\epsilon}}\int_V H_B(z,w) \abs{dw}\abs{dz}}{\int_{C_{\epsilon}}\int_{\eta} H_B(z,w)\abs{dw}\abs{dz}}.$$
Since the derivative of $H_B(\cdot,w)$ is bounded in a neighborhood of $\D$, using dominated convergence, we see
\begin{eqnarray*}
\alpha &=&\lim_{\epsilon \rightarrow 0} \frac{\int_{C_{\epsilon}}\int_V \frac{H_B(z,w)}{\epsilon} \abs{dw}\abs{dz}}{\int_{C_{\epsilon}}\int_{\eta} \frac{H_B(z,w) }{\epsilon}\abs{dw}\abs{dz}}\\
&=& \frac{\int_{C_{\epsilon}}\int_V H_{\partial B}(z,w) \abs{dw}\abs{dz}}{\int_{C_{\epsilon}}\int_{\eta} H_{\partial B}(z,w) \abs{dw}\abs{dz}}\\
&=& \frac{\mathcal{E}_B(\D,V)}{\mathcal{E}_B(\D,\eta)}.
\end{eqnarray*}
\end{proof}

\begin{proposition}
There is a unique process Feller-Dynkin process with state space $E=\C\backslash D\cup \{\D\}$ satisfying Definition \ref{characterizationERBM}.  Furthermore, this process can be defined so as to have continuous sample paths in the topology of $E$.
\end{proposition}
\begin{proof}
Propositions \ref{ERBMlikeBM}, \ref{radialpartERBM}, and \ref{excursiondistERBM} combine to show that the process defined in (\ref{ERBMdef}) satisfies Definition \ref{characterizationERBM}.  The uniqueness statement follows from Proposition \ref{semigroupERBM}.  By construction, $B_{\C \backslash \D}^{ER}$ is an $R$-process.  Using this, Propositions \ref{ERBMlikeBM} and \ref{radialpartERBM}, and the fact that Brownian motion and reflected Brownian motion have continuous sample paths, it is easy to check that the sample paths of $B_{\C \backslash \D}^{ER}$ are continuous.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ERBM IN FINITELY CONNECTED DOMAINS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Excursion Reflected Brownian Motion in Conformal Annuli}
Now let $A$ be any compact, connected subset of $\C$ larger than a single point and let
$$f: \C \backslash \D \rightarrow \C \backslash A$$
be a conformal map sending $\infty$ to $\infty$.  It is a straightforward exercise to verify that $f$ is unique up to a rotation.  Let $\sigma_t$ be the $\mathscr{F}_t$ stopping time given by
$$\int_0^{\sigma_t} \abs{f\paren{B_{\C\backslash \D}^{ER}}}^2 ds=s$$
define
$$B_{\C\backslash A}^{ER}(t)=f\paren{B_{\C \backslash D}^{ER}(t)}$$
and $\tilde{\mathscr{F}}_t=\mathscr{F}_{\sigma_t}.$
We define ERBM in $\C \backslash A$ to be the process
\begin{equation*}
B^{ER}_{\C \backslash A}:=\paren{\Omega,\mathscr{F},\{\tilde{\mathscr{F}}_t: t\geq 0\}, \{B^{ER}_{\C\backslash A}\},\{\proj^x\}}
\end{equation*}
Since $B_{\C \backslash D}^{ER}$ is rotationally invariant and $f$ is unique up to rotation, it is clear that the definition of $B_{\C\backslash A}^{ER}$ does not depend on $f$.  It is also not hard to check that the strong Markov property is preserved (see the discussion on pg. 277 of \cite{MR1796539}).  To ensure that $B_{\C\backslash A}^{ER}(t)$ exists for all time, we need to verify that
\begin{equation}
\int_0^{\sigma_t} \abs{f\paren{B_{\C\backslash \D}^{ER}}}^2 ds=\infty.
\label{ERBMalltime}
\end{equation}
In order for $B_{\C\backslash A}^{ER}(t)$ not to have a limit as $t \rightarrow \infty$, we need to verify that
\begin{equation}
\int_0^{\sigma_t} \abs{f\paren{B_{\C\backslash \D}^{ER}}}^2 ds<\infty~~\rm{a.s.}
\label{ERBMnolimit}
\end{equation}
We temporarily put these considerations aside until the next section. The first thing we check is that ERBM in conformal annuli is in fact conformally invariant.
\begin{proposition}
Suppose $f: \C \backslash \D \rightarrow A$ and $g : A \rightarrow B$ are conformal maps and $B^{ER}_A(t)$ is a reflected Brownian motion in $A$.  The process
$$B^{ER}_B(t)=B^{ER}_A(\sigma_t)$$
where
$$\int_0^{\sigma_t} \abs{g'(B^{ER}_A(s))}^2 ds=t$$
is an ERBM in $B$. \label{ERBMconformalinvariance}
\end{proposition}
\begin{proof}
Let $\sigma_r$ satisfy
$$\int_0^{\sigma_r} \abs{g'(f(B^{ER}_{\C \backslash \D}(s)))f'(B^{ER}_{\C \backslash \D}(s)}^2 ds=r$$
and define a map $T:[0,\sigma_r] \rightarrow [0, \infty]$ by
\begin{equation}
t \mapsto \int_0^t \abs{f'(B^{ER}_{\C \backslash \D}(s))}^2 ds.
\end{equation}
It is straightforward to verify that $T$ is a bijection (we use (\ref{ERBMnolimit}) here) onto $[0,T(\sigma_r)]$ with derivative $\abs{f'(B^{ER}_{\C \backslash \D}(s))}^2$.  Now by a change of variables, we have
\begin{eqnarray*}
r&=&\int_0^{\sigma_r} \abs{g'(f(B^{ER}_{\C \backslash \D}(s)))f'(B^{ER}_{\C \backslash \D}(s)}^2 ds\\
&=&\int_0^{\sigma_r} \abs{g'\paren{B^{ER}_{A}(T(s))}f'(B^{ER}_{\C \backslash \D}(s)}^2 ds\\
&=&\int_0^{T(\sigma_r)} \abs{g'(B^{ER}_{A}(s)}^2 ds.
\end{eqnarray*}
So $B^{ER}_{B}(r)=g\paren{B^{ER}_{A}(T(\sigma_r))}=g(f(B^{ER}_{\C \backslash \D}(\sigma_r)))$ and it follows that the process in $B$ defined by $g$ is the same as the process defined by $g\circ f$ and thus is an ERBM.
\end{proof}

It is now not hard to check that $B^{ER}_{\C\backslash A}$ satisfies the conditions set forth in Definition \ref{characterizationERBM}
\begin{proposition}
The process $B_{\C \backslash A}^{ER}$ satisfies Definition \ref{characterizationERBM}.
\end{proposition}
\begin{proof}
The 1st and 4th property have already been discussed.  The 2nd property follows from the conformal invariance of Brownian motion and the 3rd property follows from the conformal invariance of excursion measure (see 5.2 of \cite{MR2129588}).
\end{proof}
\begin{remark}
If $K$ is a closed subset of $\C \backslash A$ it makes sense to discuss ERBM in $\C \backslash A$ killed at $K$.  Most often we will do this when $K$ is a simple, closed curve $\eta$ surrounding $A$ and refer to the corresponding process as ERBM in $D$ where $D$ is the region bounded by $\eta$ and $\partial A$.
\end{remark}

\section{Excursion Reflected Brownian Motion in Finitely Connected Domains} \label{ERBMGeneralDef}
Let $D\in \mathcal{Y}_n$ and let $\eta_i$ for $1\leq i \leq n$ be as in Definition \ref{characterizationERBM} and denote the domain bounded by $\eta_i$ and $\partial A_i$ by $D_i$. We will now define a process $B^{ER}_D$ in $D$ satisfying Definition \ref{characterizationERBM}.  Intuitively, we define $B^{ER}_D$ pathwise to be Brownian motion up until the time it hits an $A_i$, then let it be ERBM in $D_i$ until it hits $\eta_i$, then let it be Brownian motion until it hits another $A_i$ and so on.  Adding rigor to this intuition is not hard, but is notationally cumbersome. For $i=1, \ldots n$ and $j=1,2, \ldots$ let $B_{D_i}^{(j)}$ be ERBMs in $D_i$ started at $A_i$, $B_{D_0}(t)=A_0$ for all $t$, and $B_j$ be a Brownian motion in $\C$ started at the origin.  We can construct these processes on the same probability space $\Omega$ so that they are all independent.  Now let $z \in E= D\cup\{A_0, \ldots ,A_n\}$ and define
\begin{equation*}
B^{ER}_D(t)=\begin{cases}
z & \text{if } t=0\\
A_0 & \text{if } t > \tau \\
B^{ER}_D(\sigma_j) + B_i(t-\sigma_i) & \text{if } \sigma_j < t \leq \tau_j \\
B^{(j)}_{D_i}(t-\tau_{j}) \text{ where } B^{ER}_D(\tau_j)=A_i & \text{if } \tau_j < t \leq \sigma_{j+1}
\end{cases}
\end{equation*}
where
\begin{eqnarray*}
\tau &=&\inf \{t: B^{ER}_D(t) \in A_0\}, \\
\sigma_1 &=&0, \\
\sigma_j &=& \inf \{t \geq \tau_{j-1}: B_D^{ER}(t) \in \eta_i \} \text{ for } j\geq 2, \\
\tau_j &=&  \inf \{t \geq \sigma_j: B_D^{ER}(t) \in A_i \text{ for some } i \}.
\end{eqnarray*}
For each $z$, $B_D^{ER}$ started at $z$ defines a family of probability measures $P^z_t$ indexed by $\R^+$ on $E$ (endowed with the Borel $\sigma$-algebra).  In fact, it is not hard to check that this family of probability measures defines a Feller-Dynkin $P_t$ semi-group on $E$ whose transitions are independent of the choice of the curves $\eta_i$. %\textbf{It seems like the FD statement should be standard (or at least that we are strong markov if we do this), but perhaps elaborate}


\section{A Markov Chain Associated with ERBM} \label{MarkovChainERBM}
ERBM on $D$ induces a discrete time Markov chain $X_0, X_1, \ldots$ with state space $\{A_0, \ldots A_n\}$ (see \cite{MR2247843} pg. 37).  The probability the chain moves from $A_i$ to $A_j$ is the probability that $A_j$ is the first boundary component of $D$ that $B_D^{ER}$ started at $A_i$ hits after the first time it hits $\eta_i$.  That is, the chain has transition probabilities
\begin{equation*}
p_{ij}=\int_{\eta_i} h_j(z) \frac{H_D(A_j,z)}{\mathcal{E}_{D_i}(A_i, \eta_i)} \abs{dz}
\end{equation*}
for $i\neq 1$ and $p_{00}=1$, where $h_j$ is the harmonic function on $D$ that is $1$ on $\partial A_j$ and $0$ on $\partial A_i$ for $i \neq j$ (note that $h_j(z)$ is the probability that Brownian motion in $D$ started at $z$ exits $D$ at $A_i$).  This Markov chain is not entirely satisfactory since it is highly dependent on the particular choice of $\eta_i$.  However, this chain does induce another chain with transition probabilities
\begin{equation*}
q_{ij}=\frac{p_{ij}}{1-p_{ii}}
\end{equation*}
corresponding to the transitions of $X$ the first time it visits a new site (that is, we erase all the loops).  Since $q_{j0}>0$ for all $j$, the eigenvalues of the transition matrix $Q$ have absolute value strictly less than one and, using standard results from Markov chain theory, we have that the Green's matrix
\begin{equation}\label{GreenMatrixFormula}
\mathbf{I}+\mathbf{Q}+\mathbf{Q}^2+\ldots + \mathbf{Q}^n+ \ldots=\paren{\mathbf{I}-\mathbf{Q}}^{-1}
\end{equation}
is well-defined.

